Price of Competition and Dueling Games

We study competition in a general framework introduced by Immorlica et al. and answer their main open question. Immorlica et al. considered classic optimization problems in terms of competition and introduced a general class of games called dueling games. They model this competition as a zero-sum game, where two players are competing for a user's satisfaction. In their main and most natural game, the ranking duel, a user requests a webpage by submitting a query and players output an ordering over all possible webpages based on the submitted query. The user tends to choose the ordering which displays her requested webpage in a higher rank. The goal of both players is to maximize the probability that her ordering beats that of her opponent and gets the user's attention. Immorlica et al. show this game directs both players to provide suboptimal search results. However, they leave the following as their main open question: "does competition between algorithms improve or degrade expected performance?" In this paper, we resolve this question for the ranking duel and a more general class of dueling games. More precisely, we study the quality of orderings in a competition between two players. This game is a zero-sum game, and thus any Nash equilibrium of the game can be described by minimax strategies. Let the value of the user for an ordering be a function of the position of her requested item in the corresponding ordering, and the social welfare for an ordering be the expected value of the corresponding ordering for the user. We propose the price of competition which is the ratio of the social welfare for the worst minimax strategy to the social welfare obtained by a social planner. We use this criterion for analyzing the quality of orderings in the ranking duel. We prove the quality of minimax results is surprisingly close to that of the optimum solution.

==> gen.tex <==
  \subsection{Ranking duel with general valuation}	
 \begin{proofof}{Theorem \ref{f14}}
	\input{proof1.tex}
\end{proofof}

 \subsection{Compression duel with general valuation function}\label{fu1}
\input{proof2.tex}

\subsection{Binary search duel with general valuation function}\label{fu2}
\input{proof3.tex}


==> table.tex <==
\begin{center}
    \begin{tabular}{| l | l | l | l | l | l | p{5cm} |}
    \hline
    x & $a=1$ & $a=2$ & $a=3$ & $a=4$ & $a=5$& $a=6$ &$a=6$ \\ \hline
    $b=2$ & 	0 & 0 & 0 & 0 & 0 & 0 &\\ \hline
    $b=3$ & 0 & 0 & 0 & 0 & 0 & 0 &\\ \hline
    $b=4$ & 0 & 0 & 0 & 0 & 0 & 0 &\\ \hline
    $b=5$ & 0 & 0 & 0 & 0 & 0 & 0 &\\ \hline
    $b=6$ & 0 & 0 & 0 & 0 & 0 & 0 & \\ \hline
    $b=7$ & 0 & 0 & 0 & 0 & 0 & 0 &\\ \hline
    \end{tabular}
\end{center}

==> upperbound.tex <==
\section{Upper bound for the $\POC$ of the ranking duel with linear valuation function}
\begin{theorem}
\label{fact_10}
In the linear ranking duel we have $\POC \leq 0.8334$.
\end{theorem}
\begin{proof}
Consider the following example.
Let $\Omega$ to be the set of three pages $\{a, b, c\}$, where $p_a=0.4$, $p_b=0.4$, and $p_c=0.2$. Moreover, the valuation function is defined as $f_\omega(\pi) = 3-\pi(\omega)$. Thus, $\langle a, b, c \rangle$ is the social optimum permutation. $$\SW(\OPT)=0.4\times 2 + 0.4\times 1=1.2.$$
Now consider a strategy $\xminmax$ which plays $\langle a, c, b \rangle$ and $\langle b, c, a\rangle$ with probabilities half. Table \ref{fig:uppertable} shows that the outcome of player $A$ is non-negative when he is playing strategy $\xminmax$ against all possible pure strategies. Hence, $\xminmax$ is a minmax strategy.
$$\SW(\xminmax)=\frac{\Big[0.4\times 2 + 0.2\Big] + \Big[0.4 \times 2+0.2\Big]}{2}=1.$$ Therefore, $$\POC \leq \frac{1}{1.2} \leq 0.8334.$$
\end{proof}
\begin{figure}[h]
\begin{center}
\begin{tabular}{|c|l|l|c|}
\hline
$\y$ & $u^A(\langle a,c,b \rangle,\y)$ & $u^A(\langle b,c,a \rangle,\y)$ & $u^A(\xminmax,\y)$\\
\hline
$\langle a,b,c\rangle$ &$-0.4+ 0.2=-0.2$&$-0.4+ 0.4+ 0.2=0.2$&0\\
\hline
$\langle a,c,b\rangle$ &$0$&$-0.4+ 0.4=0$&0\\
\hline
$\langle b,a,c\rangle$ &$ 0.4-0.4+ 0.2=0.2$&$-0.4+ 0.2=-0.2$&0\\
\hline
$\langle b,c,a\rangle$ &$ 0.4-0.4=0$&$0$&0\\
\hline
$\langle c,a,b\rangle$ &$ 0.4-0.2=0.2$&$-0.4+ 0.4-0.2=-0.2$&0\\
\hline
$\langle c,b,a\rangle$ &$ 0.4-0.4-0.2=-0.2$&$ 0.4-0.2=0.2$&0\\
\hline
\end{tabular}
\end{center}
\caption{Payoff of strategy $\xminmax$ against pure strategies}
\label{fig:uppertable}
\end{figure}

%%
%% End of file `elsarticle-template-1-num.tex'.
	

